Empirical Bayes Regret Minimization

Most bandit algorithm designs are purely theoretical. Therefore, they have strong regret guarantees, but also are often too conservative in practice. In this work, we pioneer the idea of algorithm design by minimizing the empirical Bayes regret, the average regret over problem instances sampled from a known distribution. We focus on a tractable instance of this problem, the confidence interval and posterior width tuning, and propose an efficient algorithm for solving it. The tuning algorithm is analyzed and evaluated in multi-armed, linear, and generalized linear bandits. We report several-fold reductions in Bayes regret for state-of-the-art bandit algorithms, simply by optimizing over a small sample from a distribution.

==> BroaderImpact.tex <==
%!TEX root = Paper.tex

\section*{Broader Impact}
\label{sec:broader impact}

Multi-armed bandits have many applications that involve users, such as search and recommender systems. In this work, we propose a tuning mechanism for existing bandit algorithms that reduces their regret. This means that the algorithms learn more efficiently, and this should be beneficial for the users that interact with them. We do not propose new applications for contextual bandits, and therefore our impact should be limited to those that already exist. We are not aware of any major societal changes that our work could cause, such as on welfare, fairness, privacy, and so on.

